VANI: Very-lightweight Accent-controllable TTS for Native and Non-native speakers with Identity Preservation

We introduce VANI, a very lightweight multi-lingual accent controllable speech synthesis system. Our model builds upon disentanglement strategies proposed in RADMMM and supports explicit control of accent, language, speaker and fine-grained $F_0$ and energy features for speech synthesis. We utilize the Indic languages dataset, released for LIMMITS 2023 as part of ICASSP Signal Processing Grand Challenge, to synthesize speech in 3 different languages. Our model supports transferring the language of a speaker while retaining their voice and the native accent of the target language. We utilize the large-parameter RADMMM model for Track $1$ and lightweight VANI model for Track $2$ and $3$ of the competition.

==> abstract.tex <==
\vspace*{-0.25\baselineskip}
In this paper, we present VANI, a very lightweight multi-lingual accent controllable speech synthesis system. Our approach builds upon RADMMM, and utilizes the same approach to create a very lightweight ($<5$ million parameters) multilingual speech model which can generate speech with the proper native accent of the target language while retaining a person's voice without relying on parallel or bilingual training with the person speaking in multiple languages. Our model supports explicit control over accent, language, speaker and fine-grained $F_0$ and energy features. We demonstrate an ability to control synthesized accent and language while retaining speakers voice in 2 settings: Indic languages dataset released for LIMMITS challenge\red{cite the challenge} with 2 speakers per language and another 7 language open-source dataset with 1 speaker per language. We examine the quality of the models and compare to large RADMMM model in terms of content, speaker retention, acoustic quality and inference speed.
\vspace*{-0.5\baselineskip}

==> conclusion.tex <==
\vspace*{-1.0\baselineskip}
We present a very-lightweight accent-controllable multilingual, multiaccented and multispeaker TTS model based on RADMMM. Our model provides an ability to predict such fine-grained features for any desired combination of speaker, accent and language. Our analysis shows ....

==> experiments.tex <==
\vspace*{-0.75\baselineskip}
We conduct our experiments on 2 data setups described below:

\subsection{Datasets}
\red{limmits icassp 2023}
\red{non parallel open source data}

\subsection{Data Pruning}
We used ASR models to prune datasets...1) TextParallel: found the maximal overlap between male and female within each language + asr cer pruning. 2) Unconstrained: ASR cer pruning.

\subsection{How different Parameter Models fare on resynthesis}

\begin{table*}[ht]
\vspace*{-0.8\baselineskip}
    \small
    % \vspace*{-1.0\baselineskip}
    % \vspace*{-0.75\baselineskip}
    \caption{[LIMMITS]Comparing model quality for resynthesis}
    \vspace{-0.8\baselineskip}
    \setlength\tabcolsep{4.0pt}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \textbf{Speaker Quality (Cosine sim)} & \textbf{Content Quality (CER)} & \textbf{Acoustic Quality(PESQ)} \\
        % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
        \midrule
        VANI-Quartznet & $0.4197 \pm 0.0149$\\
        VANI-GAN & $0.4197 \pm 0.0149$\\
        VANI-ARFlow & $0.4197 \pm 0.0149$\\
        RADMMM & $0.4197 \pm 0.0149$\\
        \midrule
        \end{tabular}
    \label{tab:data_regimes}
    
    \vspace{-1.0\baselineskip}
\label{tab:model_comparison}
\vspace{-1.0\baselineskip}
\end{table*}

\subsection{How different Parameter Models fare on transfer}

\begin{table*}[ht]
\vspace*{-0.8\baselineskip}
    \small
    % \vspace*{-1.0\baselineskip}
    % \vspace*{-0.75\baselineskip}
    \caption{[LIMMITS] Comparing model quality for language transfer}
    \vspace{-0.8\baselineskip}
    \setlength\tabcolsep{4.0pt}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \textbf{Speaker Quality (Cosine sim)} & \textbf{Content Quality (CER)} & \textbf{RTF} \\
        % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
        \midrule
        VANI-Quartznet & $0.4197 \pm 0.0149$\\
        VANI-GAN & $0.4197 \pm 0.0149$\\
        VANI-ARFlow & $0.4197 \pm 0.0149$\\
        RADMMM & $0.4197 \pm 0.0149$\\
        \midrule
        \end{tabular}
    \label{tab:data_regimes}
    
    \vspace{-1.0\baselineskip}
\label{tab:model_comparison}
\vspace{-1.0\baselineskip}
\end{table*}

\begin{table*}[ht]
\vspace*{-0.8\baselineskip}
    \small
    % \vspace*{-1.0\baselineskip}
    % \vspace*{-0.75\baselineskip}
    \caption{[NonParallel]Comparing model quality for resynthesis}
    \vspace{-0.8\baselineskip}
    \setlength\tabcolsep{4.0pt}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \textbf{Speaker Quality (Cosine sim)} & \textbf{Content Quality (CER)} & \textbf{Acoustic Quality(PESQ)} \\
        % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
        \midrule
        VANI-Quartznet & $0.4197 \pm 0.0149$\\
        VANI-GAN & $0.4197 \pm 0.0149$\\
        VANI-ARFlow & $0.4197 \pm 0.0149$\\
        RADMMM & $0.4197 \pm 0.0149$\\
        \midrule
        \end{tabular}
    \label{tab:data_regimes}
    
    \vspace{-1.0\baselineskip}
\label{tab:model_comparison}
\vspace{-1.0\baselineskip}
\end{table*}

\subsection{How different Parameter Models fare on speed}

\begin{table*}[ht]
\vspace*{-0.8\baselineskip}
    \small
    % \vspace*{-1.0\baselineskip}
    % \vspace*{-0.75\baselineskip}
    \caption{[NonParallel] Comparing model quality for language transfer}
    \vspace{-0.8\baselineskip}
    \setlength\tabcolsep{4.0pt}
    \centering
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{Speaker Quality (Cosine sim)} & \textbf{Content Quality (CER)} \\
        % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
        \midrule
        VANI-Quartznet & $0.4197 \pm 0.0149$\\
        VANI-GAN & $0.4197 \pm 0.0149$\\
        VANI-ARFlow & $0.4197 \pm 0.0149$\\
        RADMMM & $0.4197 \pm 0.0149$\\
        \midrule
        \end{tabular}
    \label{tab:data_regimes}
    
    \vspace{-1.0\baselineskip}
\label{tab:model_comparison}
\vspace{-1.0\baselineskip}
\end{table*}

\subsection{How different Parameter Models fare on quality}

\subsection{Does the data size per speaker affect quality, specially speaker identity}


% We conduct our experiments on an open source dataset\footnote{Dataset source, metadata and filelists will be released with source code.} with a sampling rate of 16kHz. It contains 7 different languages (American English, Spanish, German, French, Hindi, Brazilian Portuguese, and South American Spanish). This dataset emulates low-resource scenarios with only 1 speaker per accent with strong correlation between speaker, accent, and language. We use HiFiGAN vocoders trained individually on selected speakers in the evaluation set. % Most TTS models can synthesize good quality speech for a speaker in their own native language and accent(resynthesis). However, as our goal is to synthesize speech for a speaker in a novel target language and accent,  
% We focus on the task of transferring the voice of 7 speakers in the dataset to the 6 \emph{other} language and accent settings in the dataset. Herein we refer to RADTTS-ML as RT and RADMMM as RM for brevity.
% % \subsection{Dataset Regimes}
% % We curated two open source datasets with 16khz sampling rate. We restrict the maximum number of training samples per speaker to 10,000 for better balance across speakers in both data regimes. Dataset D1 represents the limited data regime, where we only have 1 speaker per language and hence disentanglement of speaker and accent can be more challenging. Dataset D2 represents a more relaxed situation, with multiple speakers per accent. Table \ref{tab:data_regimes} summarizes the two datasets. 

% % \begin{table}[ht]
% %     \small
% %     \vspace*{-1.0\baselineskip}
% %     \caption{Speakers and prompts in different data regimes.}
% %     \vspace*{-1.0\baselineskip}
% %     \setlength\tabcolsep{2.5pt}
% %     \centering
% %     \begin{tabular}{lcccc}
% %         \toprule
% %         \textbf{} & \multicolumn{2}{c}{\textbf{Dataset D1}} & \multicolumn{2}{c}{\textbf{Dataset D2}} \\
% %         \textbf{Language} & \textbf{Speakers} & \textbf{Prompts} & \textbf{Speakers} & \textbf{Prompts} \\
% %         \midrule
% %         English (US) & 1 & 10000 &  98 & 50199 \\
% %         German (DE) & 1 & 10000 &  6 & 58129 \\
% %         French (FR) & 1 & 10000 &  5 & 49975 \\
% %         Spanish (ES) & 1 & 10000 &  1 & 10000 \\
% %         Hindi & 1 & 9634 &  57 & 83131 \\
% %         Portuguese (BR) & 1 & 3618 &  1 & 3618 \\
% %         Spanish (LATN) & 1 & 7387 &  1 & 7387 \\
% %         Spanish (CO) & 0 & 0 & 11 & 3266 \\
% %         \midrule
% %         Total & 7 & 60639 & 180 & 265705 \\
% %         \midrule
% %         \end{tabular}
% %     \label{tab:data_regimes}
% %     \vspace{-2.0\baselineskip}
% % \end{table}

% % \subsection{Evaluation Setup}
% % % The task of re-synthesizing a speaker in their own native language with their own native accent (Resynthesis Task) is a subset of broader task of being able to synthesize the speaker in any language with target accent. Most TTS models perform well on re-synthesis in the speaker's native language~\cite{a thousand papers}. However, making a speaker speak a target language with a target accent is a challenging task, since it involves replacing the speaker's original accent with the target accent (Transfer task). In our evaluation, we focus on the Transfer task of synthesizing 7 different speakers from dataset D1 to 6 other languages (languages excluding their native language). 
% % The task of re-synthesizing a speaker in their own native language with their own native accent (Resynthesis Task) is one that most TTS models perform well on~\cite{a thousand papers}. However, making a speaker speak a target language with a target accent is a challenging task, since it involves replacing the speaker's original accent with the target accent (Transfer task). In our evaluation, we focus on the Transfer task of synthesizing 7 different speakers from dataset D1 to 6 other languages (languages excluding their native language). 

% %The criteria for evaluation involves: measuring speaker retention quality using state-of-the-art speaker recognition models like Titanet~\cite{titanet}, measure content quality using character error rate(CER) with transcripts obtained using Conformer ASR models~\cite{conformer} and human evaluations to measure accent quality. 
% \vspace*{-0.8\baselineskip}
% \subsection{Ablation of Disentanglement Strategies}
% \label{sec:ablation}
% \vspace*{-0.5\baselineskip}

% % \begin{table*}[ht]
% %     \small
% %     % \vspace*{-1.0\baselineskip}
% %     \caption{Aggregated Ablation Results.}
% %     \vspace*{-1.0\baselineskip}
% %     \setlength\tabcolsep{4.0pt}
% %     \centering
% %     \begin{tabular}{lccccc}
% %         \toprule
% %         \textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{RADTTS-ML}} & \multicolumn{2}{c}{\textbf{RADMMM}} \\
% %         \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
% %         \midrule
% %         Baseline (B) & D1 & $0.3062 \pm 0.0176$ & 17.733 & $0.3438 \pm 0.0138$ & 5.103 \\
% %         (B) + normalized $F_0$ pred & D1 & N/A & N/A & $0.3946 \pm 0.0143$ & 5.300 \\
% %         (B) + $L_{adv}$ & D1 & $0.3027 \pm 0.0174$ & 39.854 & N/A & N/A \\
% %         (B) + augmentation & D1 & $0.3855 \pm 0.0145$ & 44.302 & $ 0.2174 \pm  0.0131$ & 41.658 \\
% %         (B) + $L_{var}$ and $L_{covar}$ & D1 &  $0.4029 \pm 0.0144$ & 13.745 &  N/A & N/A \\
% %         (B) + low weight on $L_{var}$, $L_{covar}$ and $L_{cross-corr}$ & D1 &  $0.3784 \pm 0.0112$ & 16.971 & $0.3232 \pm 0.0154$ & 9.552 \\
% %         (B) + $L_{var}$, $L_{covar}$ and $L_{cross-corr}$ & D1 & $0.4217 \pm 0.0156$ & 12.224 & $0.4188 \pm 0.0148 $ & 5.481 \\
% %         (B) + $L_{var}$, $L_{covar}$, $L_{cross-corr}$ and $L_{adv}$ & D1 & N/A & N/A & $0.4163 \pm 0.0157$ & 7.172 \\
% %         \midrule
% %         \end{tabular}
% %     \label{tab:internal_ablation}
% %     % \vspace{-1.0\baselineskip}
% % \end{table*}

% % fix sizes of this later...maybe replae with plots directly from data...
% \begin{figure*}
%  \centering
%  \begin{subfigure}{0.47\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{data/radtts_ablation/RADTTS_nov3_model_combined_stats.pdf}
%     \vspace*{-1.5\baselineskip}
%     \caption{RADTTS-ML (RT)}
%     \label{fig:radtts_ablation}
% \end{subfigure}
% \begin{subfigure}{0.495\textwidth}
% \centering
%   \includegraphics[width=\linewidth]{data/radmmm_ablation/RADMMM_nov3_model_combined_stats.pdf}
%   \vspace*{-1.5\baselineskip}
%   \caption{RADMMM (RM)}
%   \label{fig:radmmm_ablation}
% \end{subfigure}
% \vspace*{-1.0\baselineskip}
% \caption{Comparing speaker cosine similarity and CER of considered disentanglement strategies for every accent.}
% \label{fig:internal_ablation_accent_wise}
% \vspace*{-1.5\baselineskip}
% \end{figure*}

% We evaluate the effects of disentanglement strategies on the transfer task by measuring speaker timbre retention using the cosine similarity (Cosine Sim) of synthesized samples to source speaker's reference speaker embeddings obtained from the speaker recognition model Titanet~\cite{titanet}. We measure character error rate (CER) with transcripts obtained from Conformer~\cite{conformer} models trained for each language. Table \ref{tab:internal_ablation} and Figure \ref{fig:internal_ablation_accent_wise} demonstrate overall and accent grouped effects of various disentanglement strategies. The \RADTTSML baseline uses the shared text token set, accent-conditioned alignment learning, and no additional constraints to disentangle speaker, text, and accent. The \RADMMM baseline uses this setup with $F_0$ and energy conditioning.
% \input{results_table}
% % \subsubsection{$L_{adv}$}
% \noindent{\textbf{Speaker Adversarial Loss ($L_{adv}$)}}
% We observe that the addition of $L_{adv}$ loss to \RADTTSML and \RADMMM does not affect speaker retention when synthesizing the speaker for a target language. However, we observe a drop in character error rate. We believe the gradients from the speaker classifier tend to remove speaker and accent information from encoded text $\Phi$, which affects the encoded text representation leading to worse pronunciation.

% % \subsubsection{Data Augmentation}
% \noindent{\textbf{Data Augmentation}}
% We use Pratt~\cite{Praat} to apply six augmentations: formant scaling down ($\times [0.875 -1.0]$) and up ($\times [1.0 - 1.25]$), scaling $F_0$ down ($\times [0.9 - 1.0]$) and up ($\times [1.0 - 1.1]$), and scaling durations to make samples faster($\times [0.9-1.0]$)) or slower($\times [1.0 -1.1]$). We augment the dataset with transformed audio defining a new speaker identifier, but retaining the original accent. In \RADTTSML, this leads to a significant boost in speaker retention. We believe that creating more speakers per accent enhances disentanglement of accent and speaker. However, in \RADMMM, where $F_0$ is predicted and the model is explicitly conditioned on augmented $F_0$, we observe a significant drop in both speaker retention as well as CER with augmentations, likely due to conditioning on noisy augmented features. %as the model is explicitly conditioned on noisy augmented features, this severely affects the synthesis quality.

% % \subsubsection{Regularization}
% \noindent{\textbf{Embedding Regularization}}
% We conduct three ablations with regularization: one that adds variance ($L_{var}$) and covariance ($L_{covar}$) constraints to the baseline, and two more involving all three constraints ($L_{var}$, $L_{covar}$, $L_{xcorr}$) with small (0.1) and large weights (10.0). We observe an improvement in speaker similarity with the best speaker retention with all three constraints in both \RADTTSML and \RADMMM. Moreover, we observe similar CER to the baselines suggesting similar pronunciation quality. 

% Our final models include regularization constraints, but we don't use augmentation and $L_{adv}$ due to worse pronunciation quality and limited success on speaker timbre retention. 
% \vspace*{-0.8\baselineskip}
% \subsection{Comparing proposed models with existing methods}
% \vspace*{-0.5\baselineskip}
% We compare our final \RADTTSML and \RADMMM with the Tacotron 2-based model described in \cite{learningfluently}, call it \TC, on the transfer task. We reproduced the model to the best of our ability, noting that training on our data was unstable, possibly due to data quality, and that results may not be representative of the original implementation. We tune denoising parameters~\cite{prenger2019waveglow} to reduce audio artifacts from \TC over-smooth generated mels~\cite{Flowtron,ren2022revisiting}. We attempted to implement YourTTS~\cite{yourtts} but ran into issues reproducing the results on our dataset and hence we don't make a direct comparison to it.

% %given that T2 produces over-smooth mel-spectrograms\cite{Flowtron,ren2022revisiting} that result in audio artifacts when vocoded, we carefully tuned the denoising parameter to reduce such artifacts.

% % % \subsubsection{Speaker identity retention}
% % \noindent{\textbf{Speaker identity retention.}}
% % Table \ref{tab:model_comparison} and Figure \ref{fig:model_comparison} demonstrates the overall and accent grouped speaker cosine similarity of our proposed models against Tacotron2 in both data regimes. We observe that RADTTS-ML and RADMMM perform at par in terms of normalized cosine similarity, however qualitatively RADMMM samples are much more clearer in both identity preservation and pronunciation. Comparing to Tacotron2, in both dataset regimes RADMMM showcases a better speaker identity retention. Since measuring pronunciation with CER and speaker retention with cosine similarity between embeddings is only a proxy for comparing model samples, we conduct a more systematic accent and speaker retention human evaluation. 

% % doesnt add much value.
% % \begin{figure}
% %  \begin{subfigure}{0.45\textwidth}
% %     \centering
% %     \includegraphics[width=\linewidth]{data/comparison_across_models/model_cosine_similarity.pdf}
% %     \vspace*{-1.5\baselineskip}
% % \end{subfigure}
% % \caption{Cosine Similarity of Synthesized speaker with GT reference across different models and data regimes.}
% % \label{fig:model_comparison}
% % \end{figure}


% % \subsubsection{Speaker identity retention}
% \noindent{\textbf{Speaker timbre retention}}
% Table \ref{tab:model_comparison} shows the speaker cosine similarity of our proposed models and \TC. We observe that both \RADTTSML and \RADMMM perform similarly in terms of speaker retention and achieve better speaker timbre retention than \TC. However, our subjective human evaluation below shows that \RADMMM samples are overall better than \RADTTSML in both timbre preservation and pronunciation.
% %Since measuring pronunciation with CER and speaker retention with cosine similarity between embeddings is only a proxy for comparing model samples, we conduct a more systematic accent and speaker retention human evaluation. 

% % removing Dataset D2 results.
% % \begin{table}[ht]
% %     \small
% %     % \vspace*{-1.0\baselineskip}
% %     \vspace*{-0.75\baselineskip}
% %     \setlength\tabcolsep{4.0pt}
% %     \centering
% %     \begin{tabular}{lccc}
% %         \toprule
% %         \textbf{Model} & \textbf{Dataset} & \textbf{Cosine Similarity} \\
% %         % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
% %         \midrule
% %         RADTTS-ML & D1 & $0.4186 \pm 0.0154$\\
% %         RADMMM & D1 & $0.4197 \pm 0.0149$\\
% %         Tacotron2 & D1 & $ 0.145 \pm 0.0119 $\\
% %         % RADMMM & D2 & $0.208 \pm 0.0118$ \\
% %         % Tacotron2 & D2 & $0.172 \pm 0.0137$\\
% %         \midrule
% %         \end{tabular}
% %     \label{tab:data_regimes}
% %     \vspace{-1.0\baselineskip}
% %     \caption{Comparing speaker quality across models}
% %     \vspace{-1.0\baselineskip}
% % \label{tab:model_comparison}
% % \end{table}


% \begin{table}[ht]
% \vspace*{-0.8\baselineskip}
%     \small
%     % \vspace*{-1.0\baselineskip}
%     % \vspace*{-0.75\baselineskip}
%     \caption{Speaker timbre retention using Cosine Sim (Sec \ref{sec:ablation})}
%     \vspace{-0.8\baselineskip}
%     \setlength\tabcolsep{4.0pt}
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         \textbf{Model} & \textbf{Cosine Similarity} \\
%         % \textbf{Disentanglement Strategy} & \textbf{Dataset} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
%         \midrule
%         RADTTS-ML (RT) & $0.4186 \pm 0.0154$\\
%         RADMMM (RM) & $0.4197 \pm 0.0149$\\
%         Tacotron2 (T2) & $ 0.145 \pm 0.0119 $\\
%         % RADMMM & D2 & $0.208 \pm 0.0118$ \\
%         % Tacotron2 & D2 & $0.172 \pm 0.0137$\\
%         \midrule
%         \end{tabular}
%     \label{tab:data_regimes}
    
%     \vspace{-1.0\baselineskip}
% \label{tab:model_comparison}
% \vspace{-1.0\baselineskip}
% \end{table}
% % \subsubsection{Accent quality human evaluation}
% % Accent is deeply coupled with pronunciation. A native speaker best suited to judging the pronunciation accuracy for their respective tongue.
% % %of a particular language can best judge if the target text was spoken with the right pronunciation that matches that of their native language. 
% % To measure the accent quality of synthesized samples, we conducted an internal study with known native speakers% within NVIDIA employees, 
% % , asking them to rate their pairwise preference between models (MOS is not suited for finer differences). Listeners were pre-
% % screened with a hearing test based on sinusoid counting and presented with a reference sample from a native speaker speaking the target text. The native speaker of the target language was also presented with a pair of synthetic samples speaking the same target text from a hidden model pair and asked to select their preferred sample in terms of pronunciation accuracy.
% \vspace*{-0.5\baselineskip}
% \subsection{Subjective human evaluation}
% \vspace*{-0.5\baselineskip}
% We conducted an internal study with native speakers to evaluate accent quality and speaker timbre retention. Raters were pre-screened with a hearing test based on sinusoid counting. Since MOS is not suited for finer differences, we use comparative mean opinion scores (CMOS) with a 5 point scale (-2 to 2) as the evaluation metric. %Each rater scores the sample quality by comparing two samples from a pair of anonymized models. A reference audio sample is provided and the criteria for rating is either accent quality or speaker's timbre quality. 
% Given a reference sample and pairs of synthesized samples from different models, the raters use the 5 point scale to indicate which sample, if any, they believe is more similar, in terms of accent or speaker timbre, to the target language pronunciation or speaker timbre in reference audio.

% \noindent{\textbf{Accent evaluation:}}
% %Accent is deeply coupled with pronunciation and native speakers are best qualified to evaluate accent.
% We conduct accent evaluation with native speakers of every language. % The raters were asked to compare samples to output closest to how a native speaker would say it. 
% Fig \ref{fig:accent_wise_cmos} shows the preference scores of native speakers with $95\%$ confidence intervals in each language for model pairs under consideration. Positive mean scores imply that the top model was preferred over the bottom model within the pair. Given limited access to native speakers, we show results for only 5 languages. We observe that there is no strong preference between \RADTTSML final and its baseline in terms of accent quality. We find similar results for \RADMMM final and its baseline, suggesting that accent and pronunciation are not compromised by our suggested disentanglement strategies. To evaluate controllable accent, we synthesize samples from our best model (\RADMMM final) for every speaker in languages other than the speaker's native language. Samples using non-native language and accent are referred to as \RADMMM final, and samples with the new language but native accent are referred to as \RADMMM accented. Raters preferred samples using the target accent (RM final) over the source speaker's accent (RM accented), indicating the effectiveness of accent transfer. Finally, \RADMMM final is preferred over \TC in terms of accent pronunciation.

% % rephrased above.
% % In order to test the effects of having controllable accent, we synthesized samples from our best model (\RADMMM final) for every speaker in the target language with target language accent and compared it against samples from same model for every speaker in target language with source speaker's original accent. We call this accented synthesis and this model as \RADMMM accented. We notice that human raters liked samples synthesized with target accent (RM final) much more over those having source speaker's original accent (RM accented) which indicates the effectiveness of the accent transfer capability in RM. Finally, \RADMMM final is preferred over \TC in terms of accent pronunciation.

% \begin{figure}
%  \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{data/subjective_evaluation/accent_mos_nov3.pdf}
%     \vspace*{-2.0\baselineskip}
% \end{subfigure}
% \caption{CMOS per accent for model pairs under consideration.}
% \label{fig:accent_wise_cmos}
% \vspace*{-1.5\baselineskip}
% \end{figure}


% % \subsubsection{Speaker identity human evaluation}
% \noindent{\textbf{Speaker timbre evaluation:}} 
% % To measure the speaker retention quality in the synthesized samples, we conducted a similar internal study within NVIDIA employees. Listeners were pre-screened with a hearing test based on sinusoid counting and presented with a reference ground truth sample from a speaker. The raters were also presented with a pair of synthetic samples for the speaker speaking the same target text from a hidden model pair. The raters were asked to select the sample that has speaker identity closer to the reference audio provided. 
% %In this test, raters were provided a reference sample demonstrating a speaker's original timbre an were asked to prefer the sample from model that is closer to the reference audio in terms of speaker timbre. 
% Table \ref{tab:cmos_results} shows CMOS scores with $95\%$ confidence intervals. First, we observe that in both \RADTTSML and \RADMMM, the final models with disentanglement strategies applied are preferred over baseline models in terms of speaker timbre retention. \RADMMM accented synthesis (RM accented) is rated as having similar speaker timbre as native accent synthesis with \RADMMM (RM final), indicating that changing accent doesn't change speaker timbre in \RADMMM, thus showcasing the disentangled nature of accent and speaker. Finally, RM final is preferred over \TC in terms of speaker timbre retention on transferring speaker's voice to target language.

% \noindent{\textbf{Effects of control with $F_0$ and $\mathcal{E}$:}} Comparing \RADMMM final with \RADTTSML final, we see that \RADMMM is preferred for most languages except German, indicating that explicit conditioning on $F_0$ and energy results in better pronunciation and accent. Moreover, as illustrated in Table \ref{tab:internal_ablation}, \RADMMM final achieves a better CER than \RADTTSML final. Table \ref{tab:cmos_results} demonstrates that explicit conditioning on $F_0$ and energy in \RADMMM results in much better speaker timbre retention compared to \RADTTSML. \RADMMM results in the best speaker retention, accent quality and pronunciation among our models.
% % \vspace*{-0.8\baselineskip}
% % \begin{table}[ht]
% %     \small
% %     % \vspace*{-1.0\baselineskip}
% %     % \vspace*{-1.0\baselineskip}
% %     \setlength\tabcolsep{1.5pt}
% %     \centering
% %     \begin{tabular}{lcc}
% %         \toprule
% %         \textbf{Model Pair} & \textbf{Speaker Preference} & \textbf{Accent Preference} \\
% %         \midrule
% %         RT Final vs RT Base & $0.300 \pm 0.200 $ & $0.124 \pm 0.376$ \\
% %         RM Final vs RM Base & $0.750 \pm 0.189 $ & $-0.072 \pm 0.410$ \\
% %         RM Final vs RT Final & $0.733 \pm 0.184$ & $0.676 \pm 0.348$ \\
% %         RM Final vs RM Accented & $0.025 \pm 0.199$ & $0.738 \pm 0.373$ \\
% %         RM Final vs T2 & $1.283 \pm 0.144$ & $1.144 \pm 0.320$ \\
% %         \midrule
% %         \end{tabular}
% %  \vspace{-1.0\baselineskip}
% % \caption{CMOS for speaker timbre and accent evaluation.}
% % \vspace{-1.0\baselineskip}
% % \label{tab:cmos_results}
% % \end{table}

% \vspace*{-0.8\baselineskip}
% \begin{table}[ht]
%     \small
%     % \vspace*{-1.0\baselineskip}
%     % \vspace*{-1.0\baselineskip}
%     \caption{CMOS for speaker timbre similarity.}
%     \vspace{-1.0\baselineskip}
%     \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{lc}
%         \toprule
%         \textbf{Model Pair} & \textbf{CMOS} \\
%         \midrule
%         RT Final vs RT Base & $0.300 \pm 0.200 $ \\
%         RM Final vs RM Base & $0.750 \pm 0.189 $ \\
%         RM Final vs RT Final & $0.733 \pm 0.184$ \\
%         RM Final vs RM Accented & $0.025 \pm 0.199$ \\
%         RM Final vs T2 & $1.283 \pm 0.144$ \\
%         \midrule
%         \end{tabular}
% %  \vspace{-1.0\baselineskip}

% \label{tab:cmos_results}
% \vspace{-1.0\baselineskip}
% \end{table}

% \vspace{-1.0\baselineskip}

==> introduction.tex <==
\vspace*{-0.75\baselineskip}
Recent progress in Text-To-Speech (TTS) has achieved human-like quality in synthesized mel-spectrograms ~\cite{Tacotron, Tacotron2, Flowtron, rad_tts} and waveforms~\cite{NaturalSpeech, kim2021vits}. Most models support speaker selection during inference by learning a speaker embedding table~\cite{Tacotron, Tacotron2, Flowtron} during training, while some support zero-shot speaker synthesis by generating a speaker conditioning vector from a short audio sample~\cite{speakerverificationtransfer}. However, most models support only a single language. Moreover, most of these models require a lot of parameters. \red{parameter details of past big models}, and part of our goal is to have a lightweight model that can even be deployed on end surfaces....

It is very expensive to obtain bilingual datasets because most speakers are unilingual. Hence, speaker, language, and accent attributes are highly correlated in most TTS datasets. Training models with such entangled data can result in poor language, accent and speaker transferability. RADMMM proposed several modifications to the TTS pipeline that help disentangle speaker, language and accent with fine-grained control over $F0$ and energy features. Moreover, the shared alphabet setup and online alignment mechanism of RADMMM supports scaling to any new language. 

In this work, we \textbf{(1)} demonstrate effective scaling of RADMMM setup to multiple new languages. \textbf{(2)} factorize accent, speaker and provide an ability to control the synthesized accent and language for selected speaker; \textbf{(3)} explore several generative and discriminative formulations for the TTS decoder with the above factorization. \textbf{(4)} develop several lightweight TTS models and examine their quality against the large RADMMM model in terms of content,
speaker retention, acoustic quality and inference speed.
 
\vspace*{-1.0\baselineskip}

==> method.tex <==
\vspace*{-0.75\baselineskip}
We build upon the strategies proposed in RADMMM~\cite{rad_tts,radpp} to develop a lightweight multilingual TTS system.  Our model synthesizes mels($X \in \mathbb{R}^{C_{\mathit{mel}} \times F}$) using encoded text($\Phi \in \mathbb{R}^{C_{\mathit{txt}} \times T}$), accent($A \in \mathbb{R}^{D_{\mathit{accent}}}$), speaker($S \in \mathbb{R}^{D_{\mathit{speaker}}}$), fundamental frequency($F_0 \in \mathbb{R}^{\mathit{1} \times F}$) and energy($\xi \in \mathbb{R}^{\mathit{1} \times F}$) as conditioning variables where $F$ is the number of mel frames, $T$ is the text length, and energy is per-frame mel energy average. Fig \red{add overview figure} demonstrates the setup. 

\begin{multline}
P_{vani}(X, \Lambda) = P_{mel}(X | \Phi, \Lambda, A, S, F_0, \mathcal{E})\\
P_{F_0}(F_0 | \Phi, A, S) P_{\mathcal{E}}(\mathcal{E} | \Phi, A, S) P_{dur}(\Lambda | \Phi, A, S)
\end{multline}

We leverage the text preprocessing, shared alphabet set and the accent-conditioned alignment learning mechanism proposed in RADMMM to our setup. This supports code-switching by default and allows for having a single model that works with many languages. We consider language to be \emph{implicit in the phoneme sequence} and the sequence of IPA tokens carry this information whereas the information captured by accent variable $A$ should explain the fine-grained differences between \emph{how phonemes are pronounced in different languages}.

\vspace*{-0.8\baselineskip}
\subsection{Deterministic Decoder}
\vspace*{-0.5\baselineskip}
details....deterministic decoders tend to produce oversmoothed mels.

\subsection{Generative Decoder with adversarial training}
details....still produces oversmoothed mels.

\subsection{Autoregressive Flow based decoder}
details...cleaner mels...maybe use PESQ to showcase quality.

\subsection{Attribute Predictors}
Following \cite{radpp}, we train deterministic attribute predictors to predict phoneme durations $\Lambda$, $F_0$, and energy $\mathcal{E}$ conditioned on speaker $S$, encoded text $\Phi$, and accent $A$.



% \noindent{\textbf{Data Augmentation for overfitting}}
% Disentangling accent and speaker is challenging, as a speaker typically has a specific way of pronouncing words and phonemes, causing a strong association between speaker and accent. Straightforward approaches to learning from non-parallel data learn entangled representations because a speaker's language and accent can be trivially learned from the dataset. Since our goal is to synthesize speech for a speaker in a target language with desired accent, disentangling speaker $S$ and accent $A$ is essential, otherwise either speaker identity is not preserved in the target language or the generated speech retains the speaker's accent from the source language. To overcome this problem, we use data augmentations like formant, $F_0$, and duration scaling to promote disentanglement between speaker and accent. For a given speech sample $x_i$ with speaker identity $s_i$ and accent $a_i$, we apply a fixed transformation $t \in \{1, 2, ... \tau\}$ to construct a transformed speech sample $x_i^{t}$ and assign speaker identity as $s_i + t \cdot N_{speakers}$ and accent as original accent $a_i$, where $\tau$ is the number of augmentations. This creates speech samples with variations in speaker identity and accent in order to orthogonalize these attributes. 



==> old_apm_metrics_table.tex <==
\begin{table*}[h]
\caption{\label{tab:vanimetrics}Evaluation of models with speaker identity match using Cosine Sim and content quality using CER}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    Model & \multicolumn{2}{|c|}{Hindi Female} & \multicolumn{2}{|c|}{Hindi Male} &  \multicolumn{2}{|c|}{Marathi Female} & \multicolumn{2}{|c|}{Marathi Male} & \multicolumn{2}{|c|}{Telugu Female} & \multicolumn{2}{|c|}{Telugu Male} & \hline

         ~ & Cosine Sim & CER & Cosine Sim & CER & Cosine Sim & CER & Cosine Sim & CER & Cosine Sim & CER & Cosine Sim & CER\\ \hline
         &  &  & &  &  & & & &  & &  & \\ 
        Track1 (RADMMM) & $ 0.897 \pm 0.016 $ & 0.089 & $ 0.880 \pm 0.016 $ & 0.054 & $ 0.811 \pm 0.056 $ & 0.138 & $ 0.883 \pm 0.015 $ & 0.118 & $ 0.853 \pm 0.047 $ & 0.76 & $ 0.868 \pm 0.030 $ & 0.074\\ \hline 
         &  &  & &  &  & & & &  & &  & \\ 
        Track2 (VANI-NP) & $ 0.853 \pm 0.037 $ & 0.134 & $ 0.789 \pm 0.035 $ & 0.118 & $ 0.748 \pm 0.039 $ & 0.228 & $ 0.778 \pm 0.030 $ & 0.249 & $ 0.736 \pm 0.070 $ & 0.187 & $ 0.748 \pm 0.037 $ & 0.233 \\ \hline 
         &  &  & &  &  & & & &  & &  & \\ 
        Track3 (VANI-P) & $ 0.842 \pm 0.026 $ & 0.146 & $ 0.741 \pm 0.037 $ & 0.119 & $ 0.710 \pm 0.037 $ & 0.281 & $ 0.739 \pm 0.035 $ & 0.268 & $ 0.704 \pm 0.077 $ & 0.280 & $ 0.69 \pm 0.042 $ & 0.305 \\ 
        
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> results_table.tex <==
% \begin{table*}[h]
%     \small
%     % \vspace*{-1.0\baselineskip}
%     \caption{Aggregated Ablation Results.}
%     \vspace*{-1.0\baselineskip}
%     \setlength\tabcolsep{4.0pt}
%     \centering
%     \begin{tabular}{lcccc}
%         \toprule
%         \textbf{} & \multicolumn{2}{c}{\textbf{RADTTS-ML}} & \multicolumn{2}{c}{\textbf{RADMMM}} \\
%         \textbf{Disentanglement Strategy} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
%         \midrule
%         Baseline (B) & $0.3062 \pm 0.0176$ & 17.733 & $0.3438 \pm 0.0138$ & 5.103 \\
%         (B) + normalized $F_0$ pred & N/A & N/A & $0.3946 \pm 0.0143$ & 5.300 \\
%         (B) + $L_{adv}$ & $0.3027 \pm 0.0174$ & 39.854 & N/A & N/A \\
%         (B) + augmentation & $0.3855 \pm 0.0145$ & 44.302 & $ 0.2174 \pm  0.0131$ & 41.658 \\
%         (B) + $L_{var}$ and $L_{covar}$ &  $0.4029 \pm 0.0144$ & 13.745 &  N/A & N/A \\
%         (B) + low weight on $L_{var}$, $L_{covar}$ and $L_{cross-corr}$ &  $0.3784 \pm 0.0112$ & 16.971 & $0.3232 \pm 0.0154$ & 9.552 \\
%         (B) + $L_{var}$, $L_{covar}$ and $L_{cross-corr}$ & $0.4217 \pm 0.0156$ & 12.224 & $0.4188 \pm 0.0148 $ & 5.481 \\
%         (B) + $L_{var}$, $L_{covar}$, $L_{cross-corr}$ and $L_{adv}$ & N/A & N/A & $0.4163 \pm 0.0157$ & 7.172 \\
%         \midrule
%         \end{tabular}
%     \label{tab:internal_ablation}
%     \vspace{-0.5\baselineskip}
% \end{table*}

% \vspace{-0.8\baselineskip}
\begin{table}[!ht]
\vspace*{-0.8\baselineskip}
\caption{Ablation results comparing disentanglement strategies using Cosine Sim and CER defined in \ref{sec:ablation}}
\label{tab:internal_ablation}
\vspace*{-0.8\baselineskip}
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{lcccc}
        \toprule
        \textbf{} & \multicolumn{2}{c}{\textbf{RADTTS-ML}} & \multicolumn{2}{c}{\textbf{RADMMM}} \\
        \textbf{Disentanglement Strategy} & \textbf{Cosine Sim} & \textbf{CER} & \textbf{Cosine Sim} & \textbf{CER} \\
        \midrule
        Baseline (B) & $0.3062 \pm 0.0176$ & 17.7 & $0.3438 \pm 0.0138$ & 5.1 \\
        (B) + normalized $F_0$ pred & N/A & N/A & $0.3946 \pm 0.0143$ & 5.3 \\
        (B) + $L_{adv}$ & $0.3027 \pm 0.0174$ & 39.9 & N/A & N/A \\
        (B) + augmentation & $0.3855 \pm 0.0145$ & 44.3 & $ 0.2174 \pm  0.0131$ & 41.7 \\
        (B) + $L_{var}$ and $L_{covar}$ &  $0.4029 \pm 0.0144$ & 13.7 &  N/A & N/A \\
        (B) + low weight on $L_{var}$, $L_{covar}$ and $L_{xcorr}$ &  $0.3784 \pm 0.0112$ & 17.0 & $0.3232 \pm 0.0154$ & 9.6 \\
        (B) + $L_{var}$, $L_{covar}$ and $L_{xcorr}$ & $0.4217 \pm 0.0156$ & 12.2 & $0.4188 \pm 0.0148 $ & 5.5 \\
        (B) + $L_{var}$, $L_{covar}$, $L_{xcorr}$ and $L_{adv}$ & N/A & N/A & $0.4163 \pm 0.0157$ & 7.2 \\
        \midrule
        \end{tabular}
}

\vspace{-0.8\baselineskip}
\label{tab:internal_ablation}
\end{table}

==> table_track1.tex <==
\begin{table}[h]
\caption{\label{tab:metrics1}Summary of the objective metrics.}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \resizebox{\columnwidth}{!}{\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
    speaker & \multicolumn{2}{|c|}{transfer}& \multicolumn{3}{|c|}{resynthesis}&  \multicolumn{3}{|c|}{ground truth}& \hline

         ~ & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL \\ \hline
        hi_f & ~ & 6.7 & ~ & 8.9 & ~ & ~ & 7 & ~ \\ \hline
        hi_m & ~ & 5.7 & ~ & 5.4 & ~ & ~ & 5.3 & ~ \\ \hline
        mr_f & ~ & 14.7 & ~ & 11.86 & ~ & ~ & 12 & ~ \\ \hline
        mr_m & ~ & 16.7 & ~ & 13.8 & ~ & ~ & 11 & ~ \\ \hline
        te_f & ~ & 7.7 & ~ & 7.4 & ~ & ~ & 7 & ~ \\ \hline
        te_m & ~ & 8.6 & ~ & 7.6 & ~ & ~ & 7 & ~ \\ \hline
        
    \bottomrule
    \end{tabular}}
    \end{adjustbox}
\end{table}

==> table_track2.tex <==
\begin{table}[h]
\caption{\label{tab:metrics1}Summary of the objective metrics.}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \resizebox{\columnwidth}{!}{\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
    speaker & \multicolumn{2}{|c|}{transfer}& \multicolumn{3}{|c|}{resynthesis}&  \multicolumn{3}{|c|}{ground truth}& \hline

         ~ & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL \\ \hline
        hi_f & ~ & 6.7 & ~ & 8.9 & ~ & ~ & 7 & ~ \\ \hline
        hi_m & ~ & 5.7 & ~ & 5.4 & ~ & ~ & 5.3 & ~ \\ \hline
        mr_f & ~ & 14.7 & ~ & 11.86 & ~ & ~ & 12 & ~ \\ \hline
        mr_m & ~ & 16.7 & ~ & 13.8 & ~ & ~ & 11 & ~ \\ \hline
        te_f & ~ & 7.7 & ~ & 7.4 & ~ & ~ & 7 & ~ \\ \hline
        te_m & ~ & 8.6 & ~ & 7.6 & ~ & ~ & 7 & ~ \\ \hline
        
    \bottomrule
    \end{tabular}}
    \end{adjustbox}
\end{table}

==> table_track3.tex <==
\begin{table*}[h]
\caption{\label{tab:metrics3}Summary of the objective metrics.}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
    speaker & \multicolumn{2}{|c|}{transfer}& \multicolumn{3}{|c|}{resynthesis}&  \multicolumn{3}{|c|}{ground truth}& \hline

         ~ & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL & \multicolumn{1}{|p{1cm}|}{Cosine Sim} & CER & VisQOL \\ \hline
        hi_f & ~ & 6.7 & ~ & 8.9 & ~ & ~ & 7 & ~ \\ \hline
        hi_m & ~ & 5.7 & ~ & 5.4 & ~ & ~ & 5.3 & ~ \\ \hline
        mr_f & ~ & 14.7 & ~ & 11.86 & ~ & ~ & 12 & ~ \\ \hline
        mr_m & ~ & 16.7 & ~ & 13.8 & ~ & ~ & 11 & ~ \\ \hline
        te_f & ~ & 7.7 & ~ & 7.4 & ~ & ~ & 7 & ~ \\ \hline
        te_m & ~ & 8.6 & ~ & 7.6 & ~ & ~ & 7 & ~ \\ \hline
        
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}
